OpenCodeInterpreter: Integrating Code Generation with Execution and Refinement

The introduction of large language models has significantly advanced code generation. However, open-source models often lack the execution capabilities and iterative refinement of advanced systems like the GPT-4 Code Interpreter. To address this, we introduce OpenCodeInterpreter, a family of open-source code systems designed for generating, executing, and iteratively refining code. Supported by Code-Feedback, a dataset featuring 68K multi-turn interactions, OpenCodeInterpreter integrates execution and human feedback for dynamic code refinement. Our comprehensive evaluation of OpenCodeInterpreter across key benchmarks such as HumanEval, MBPP, and their enhanced versions from EvalPlus reveals its exceptional performance. Notably, OpenCodeInterpreter-33B achieves an accuracy of 83.2 (76.4) on the average (and plus versions) of HumanEval and MBPP, closely rivaling GPT-4's 84.2 (76.2) and further elevates to 91.6 (84.6) with synthesized human feedback from GPT-4. OpenCodeInterpreter brings the gap between open-source code generation models and proprietary systems like GPT-4 Code Interpreter.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/dataset.tex <==
\section{\dataset}

% multi-turn execute feedback
    % respond and make correction according to previous erroneous outputs
    % let GPT-4 determine whether continue or not
% multi-turn user feedback
    % user simulator: generate user feedback with GPT-4
    % generate code with given user feedback
% execute feedback distribution (#turns)
% user feedback distribution (#turns)
% programming language distribution (#queries)

\begin{figure*}[!t]
    \centering
\includegraphics[width=\linewidth]{figures/code_interpreter_data_collection.pdf}
    \caption{Data collection process: including multi-turn execution feedback and multi-turn user feedback. }
\label{fig:data_collection}
    \vspace{-3ex}
\end{figure*}

%Constructing the training data for self-correction and revision in response to user feedback involves a multi-faceted approach. 
This subsection details the methods employed for data collection, focusing on capturing diverse, real-world interactions that simulate the feedback loop between users and the model. 
The goal is to create a dataset that enables the model to learn how to respond, make corrections based on previous outputs, and determine when to continue a conversation or interaction. 
As shown in Figure \ref{fig:data_collection}, the data collection process is divided into two components: multi-turn execution feedback and multi-turn human feedback. 
All prompts used in data collection are in \ref{sec:prompt_used_in_data_collection}.
Data statistics are shown in Table ~\ref{tab:Data_Statistics}.

\begin{table}[t]
\renewcommand\tabcolsep{2.5pt}
\renewcommand\arraystretch{1.12}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
Category & Size & \begin{tabular}[c]{@{}c@{}}Human\\ -Feedback\end{tabular}  &     \begin{tabular}[c]{@{}c@{}}Exec.\\ -Feedback\end{tabular}  &   \begin{tabular}[c]{@{}c@{}}Multi\\ -Round\end{tabular}   \\
\midrule
Single Round & 111K & \redmark & \redmark & \redmark \\\midrule
LeetCode & 0.5K & \greencheck & \redmark & \greencheck \\
Code Correction & 0.5K & \redmark & \greencheck & \greencheck \\
Single Round Packing & 16K & \greencheck & \redmark & \greencheck \\
User Simulation & 51K & \greencheck & \greencheck & \greencheck \\ \hdashline
\quad Total & 68K & \greencheck & \greencheck & \greencheck \\

 \bottomrule
\end{tabular}
}
\caption{Statistics of \dataset.}

% The acronyms Single Round, LeetCode, Code Correction, User Simulation, and Single Round Patching represent LeetCode-Chain-based Multi-Round Data, Code Correction Catalyst Data, User Simulator-based Multi-Round Data, Neighbor-Document-based Synthetic Multi-Round Data, and High-Quality Single-Turn Data, respectively.}

\label{tab:Data_Statistics}
\vspace{-5mm}
\end{table}

\subsection{Code Query Selection}
We carefully initialize the source single-round data seed as a composition of Magicoder~\cite{wei2023magicoder}, python code subset of ShareGPTMagicoder-Evol-Instruct and Evol-Instruct-Code 
%\footnote{\url{https://huggingface.co/datasets/ajibawa-2023/Python-Code-23k-ShareGPT}}, 
%\footnote{\url{https://huggingface.co/datasets/ise-uiuc/Magicoder-Evol-Instruct-110K}}, 
%\footnote{\url{https://huggingface.co/datasets/nickrosh/Evol-Instruct-Code-80k-v1}}
to cover diverse high-quality 
code generation instructions
%\footnote{Nota bene that both Magicoder-Evol-Instruct and Evol-Instruct-Code are unofficial implementations of WizardCoder~\cite{luo2023wizardcoder} with different data distribution since WizardCoder doesn't release its data.}.
To further select the most informative and complex instructions from the seed set, we propose a two-stage data filtering procedure based on Qwen-72B~\cite{bai2023qwen} to process our seed dataset.
\begin{itemize}
    \item \textbf{Coarse-grained Filtering:} We ask LLM to rate the code queries and related codes in the seed set on a scale of 1 to 5 based on their complexity.
    We only retain the code queries, scoring 4 and 5, i.e. the hardest subset, in the seed set. The detailed prompt refers to {Appendix~\ref{sec:prompt_used_in_data_collection}}.
    \item \textbf{Fine-grained Filtering:} We ask LLM to rate the code queries and related codes in the seed set after the first stage on a scale of 1 to 5 based on their complexity.
    1 represents that the code query is moderately difficult, while 5 represents that the code query is an expert-level requirement.
    The detailed prompt refers to {Appendix~\ref{sec:prompt_used_in_data_collection}}.

\end{itemize}

We prepare 145k high-quality single-round code instructions after the source data filtering.
The statistics are detailed in \textcolor{red}{Appendix~\ref{}}.

\subsection{Multi-Turn Execution Feedback}
\label{sec:execution_feedback}
This part focuses on gathering data from interactions where the model is required to respond and make corrections according to its previous outputs. The process is iterative and aims to mimic real-world scenarios where a user might point out errors or request clarifications on the model's responses. To achieve this, the following steps are employed:

\begin{itemize}
    \item \textbf{Initial Interaction Collection:} Interactions are initiated with a set of predefined prompts that cover a broad spectrum of programming languages, scenarios and requirements. These prompts may elicit responses from the model that can potentially contain errors or ambiguities.
    \item \textbf{Feedback Generation:} We then extracted the code snippets from the response and executed them in a sandbox environment. The execution results will be appended to the end of dialog history and sent to GPT-4, and we let GPT-4 determine the next action. If GPT-4 considers the results to be correct, the feedback process is finished. Otherwise, we asked GPT-4 to regenerate a new version of the code until the results are correct. This iterative feedback process mimics the actual debug process of human programmers, where we often make corrections according to execution results.
\end{itemize}

It is worth noting that to align with the multi-turn human feedback introduced later, we added the prefix "Execution result: " before the actual execution output as indicators for our models.

\subsection{Multi-Turn Human Feedback}
The second component of the data collection process involves the creation of a user simulator that generates feedback for the model's responses.
We devise four methodologies to construct multi-turn human feedback datasets aimed at instructing code generation models in iterative learning based on such feedback.
This part focuses on the intuitions and details of the four methodologies:

\noindent\textbf{Single Round Patching.} Drawing on the concept of in-context pretraining~\citep{shi2023context}, we amalgamate similar single-round query-response pairs to construct multi-round dialogues.
To achieve this, we adopt the BERT-base~\cite{devlin2018bert} embedding method for transforming queries into vector representations. 
For each query, we then apply the $k$-nearest neighbors algorithm to pinpoint the five most closely related queries. 


We sequentially align each single-round instruction with two or three of its closest neighbors to create multi-round data, ensuring that each single-round instruction appears only once in the final synthetic dataset.
We finally concatenate these related single-round instructions as multi-round synthetic instances.
Through neighbor-document-based data augmentation, we generate 16.6k multi-round synthetic instances.


\paragraph{LeetCode}
Taking inspiration from the common practice among human programmers who often master a shared knowledge base by solving similar LeetCode problems, we extract similar LeetCode questions and their corresponding solutions from the LeetCode dataset in TACO~\cite{li2023taco}.
LeetCode\footnote{\url{https://leetcode.cn/problemset/}} tags related questions in their UI, allowing us to easily extract the related questions.
TACO verifies that the LeetCode dataset has been decontaminated to avoid influencing the performance of HumanEval and MBPP.
By concatenating related LeetCode questions, we generate a total of 303 multi-round instances.
Additionally, we parse the solutions in the LeetCode dataset to extract solutions of the same LeetCode questions with different time or space complexity or using different programming languages.
By concatenating different solutions to the same LeetCode questions, we generate a total of 200 multi-round instances.
Subsequently, all LeetCode-Chain-based multi-round instances undergo further rephrasing by GPT-4 to ensure alignment with the typical feedback patterns of human programmers.



\paragraph{User Simulator-based Multi-Round Data}
Successful multi-round collaborative coding necessitates more diverse interaction data. We propose a two-step data collection process focusing on creating a user simulator based on GPT-4 for generating feedback on model responses. This user simulator is designed to mimic real user feedback in multi-turn conversations. Firstly, in order to keep balance between the diversity and effectiveness of generated human feedback, we frame the human feedback data to cover a wide range of areas including syntax and formatting, efficiency, functionality enhancements, code clarity and documentation, bug identification, security improvements, compatibility and testing, resource optimization, scalability, and adherence to best practices. Each category aims to improve the quality and functionality of the code by addressing specific aspects such as performance optimization, feature enhancement, and maintainability. The details of each type of feedback are illustrated in Appendix \ref{}. Then, we utilize GPT-4 to generate human feedback with structured reasoning, which enables the simulator to generate diverse and human-like feedback. Specifically, this process involves GPT-4 assessing the code to identify satisfactory and improvable aspects, focusing on a specific area for feedback, and generating relevant human feedback accordingly. This structured reasoning process is designed to enhance the model's ability to critically analyze and iteratively refine its outputs based on the feedback. Finally, the user simulator appends generated feedback to the dialog history, prompting GPT-4 to generate solutions that address the feedback requirements. This simulates complex user-model interactions, along with interleaving multi-turn execution feedback loops introduced in Section \ref{sec:execution_feedback}, where GPT-4 also makes self-corrections based on the human feedback to improve the proposed solutions.

\paragraph{Code Correction Catalyst Data} 
In order to enhance the model's robustness, an additional step was incorporated into our data collection process, focusing on the creation of 500 specific error correction interactions. Specifically, we engineered scenarios where GPT-4 was prompted to deliberately generate incorrect code snippets. Following this, the model utilized the error messages resulting from the execution of these incorrect codes as a basis for making corrections. This approach not only simulates a realistic coding environment where programmers iteratively debug and refine their code but also enriches our dataset with a wide range of error-handling examples. During training, the instructions that originally prompted the generation of incorrect code were replaced with commands aimed at producing correct code outputs. This methodology ensures that the model learns not only from accurate code generation tasks but also gains the ability to identify and correct errors, thereby significantly improving its problem-solving capabilities and understanding of the debugging process.

% The second component of the data collection process involves the creation of a user simulator that generates feedback for the model's responses. This simulator is built on GPT-4 and is designed to act like a real user providing feedback in a multi-turn conversation. The steps for this process include:

% \begin{enumerate}
%    \item \textbf{human feedback Framing:} We carefully designed ten types of feedback for GPT-4 to refer to. Including:
%    \begin{itemize}
%        \item Syntax and Formatting: Checking for syntax errors, inconsistent formatting, and suggesting adherence to standard coding styles for readability and maintainability.
%        \item Efficiency: Identifying parts of the code that can be optimized for better performance, such as reducing time complexity, optimizing loops, or suggesting more efficient data structures.
%        \item Functionality Enhancements: Suggesting additional features or enhancements that could make the code more functional or user-friendly.
%        \item Code Clarity and Documentation: Recommending improvements in code comments and documentation to make the code more understandable and easier to maintain.
%        \item Bug Identification: Pointing out any potential bugs or logical errors in the code and suggesting ways to fix them.
%        \item Security Improvements: Highlighting any security vulnerabilities in the code and suggesting best practices to enhance security.
%        \item Compatibility and Testing: Advising on making the code more compatible with different environments or platforms and suggesting more comprehensive testing scenarios.
%        \item Resource Optimization: Identifying areas where the code might be using more resources than necessary (like memory or CPU) and suggesting optimizations.
%        \item Scalability: Providing insights on how the code can be made more scalable to handle larger data sets or more users
%        \item Adherence to Best Practices: Ensuring the code follows the best practices specific to the language or framework being used.
%    \end{itemize}
%    \item \textbf{Generating human feedback with Multi-step Reasoning:} We then built a multi-step reasoning pipeline to generate diverse and human-like user feedback. 
%    Firstly, we will enable GPT-4 to assess the current code to determine which aspects have been satisfactorily addressed. 
%    Following this evaluation, GPT-4 will identify potential areas for improvement within the code. 
%    Subsequently, it will select one of these areas to focus on as the final feedback type. 
%    For each iteration, GPT-4 itself will decide which type of feedback to use and generate the specific user feedback accordingly. 
%    This approach aims to enhance the model's ability to critically analyze its outputs and iteratively refine them based on a structured reasoning process.
%\end{enumerate}

% We append the generated user feedback to the dialog history and ask GPT-4 to generate a proper solution to fulfill requirements in these feedback. To simulate complex interactions between the users and models, the user feedback process may also repeat multiple times. It is worth noting that multi-turn execute feedback is also applied to this step, which means that GPT-4 still makes self-corrections when trying to make improvements according to the user feedback.
